Saturating Sorting without Sorts

We present a first-order theorem proving framework for establishing the correctness of functional programs implementing sorting algorithms with recursive data structures. We formalize the semantics of recursive programs in many-sorted first-order logic and integrate sortedness/permutation properties within our first-order formalization. Rather than focusing on sorting lists of elements of specific first-order theories, such as integer arithmetic, our list formalization relies on a sort parameter abstracting (arithmetic) theories and hence concrete sorts. We formalize the permutation property of lists in first-order logic so that we automatically prove verification conditions of such algorithms purely by superpositon-based first-order reasoning. Doing so, we adjust recent efforts for automating inducion in saturation. We advocate a compositional approach for automating proofs by induction required to verify functional programs implementing and preserving sorting and permutation properties over parameterized list structures. Our work turns saturation-based first-order theorem proving into an automated verification engine by (i) guiding automated inductive reasoning with manual proof splits and (ii) fully automating inductive reasoning in saturation. We showcase the applicability of our framework over recursive sorting algorithms, including Mergesort and Quicksort.

==> implementation.tex <==
\section{Implementation}\label{sec:impl}

Vampire + structural and computation induction

smtlib recursive sorting algorithms taken from the book 


==> interproc.tex <==
\section{Interprocedural Analysis}


==> invgen.tex <==
\section{Invariant Extraction}

